Protecting the Grid against IoT Botnets of High-Wattage Devices

We provide methods to prevent line failures in the power grid caused by a newly revealed MAnipulation of Demand (MAD) attacks via an IoT botnet of high-wattage devices. In particular, we develop two algorithms named Securing Additional margin For generators in Economic dispatch (SAFE) Algorithm and Iteratively MiniMize and boUNd Economic dispatch (IMMUNE) Algorithm for finding robust operating points for generators during the economic dispatch such that no lines are overloaded after automatic primary control response to any MAD attacks. In situations that the operating cost of the grid in a robust state is costly (or no robust operating points exist), we provide efficient methods to verify--in advance--if possible line overloads can be cleared during the secondary control after any MAD attacks. We then define the $\alpha D$-robustness notion for the grids indicating that any line failures can be cleared during the secondary control if an adversary can increase/decrease the demands by $\alpha$ fraction. We demonstrate that practical upper and lower bounds on the maximum $\alpha$ for which the grid is $\alpha D$-robust can be found efficiently in polynomial time. Finally, we evaluate the performance of the developed algorithms and methods on realistic power grid test cases. Our work provides the first methods for protecting the grid against potential line failures caused by MAD attacks.

==> Sources/left_overs.tex <==



%\section{Hardness}
%\emph{Defender problem:} Given $p_1,p_2,\dots,p_k$ and $\alpha$, is there operating points $p_{k+1},\dots,p_n$ for the generators such that no lines will be overloaded after any attack such that $\forall i\leq k: -\alpha p_i\leq\Delta p_i\leq\alpha p_i$?
%\vspace*{0.2cm}
%
%It is easy to see that the defender problem is in NP.





 \iffalse
\section{Unit Commitment}

As discussed in the previous subsection, in order to avoid line failures, the grid operator needs to solve optimization (\ref{eq:ec_dis}) or use the IMMUNE Algorithm for dispatching the generation. If (\ref{eq:ec_dis})--or in the case of the IMMUNE Algorithm (\ref{eq:ec_dis2})--is not feasible, however, the generation cannot be dispatched securely. Hence, in the unit commitment phase, in addition to commit enough units to have $\sum_{i=k+1}^n \overline{p_i}>-\sum_{l=1}^k (p_l-\Delta p_l^{\text{max}})$, the grid operator needs to make sure that (\ref{eq:ec_dis}) or (\ref{eq:ec_dis2}) will be feasible in the hourly dispatching.

Since the unit commitment problem is a combinatorial problem, finding a polynomial time algorithm for unit commitment is impossible unless $P=NP$~\cite{tseng2000solving}. According to~\cite[Chapter 4]{wood2012power}, many of the large market operators in the United States now use integer programming solvers to perform the unit commitment calculation. Hence, the extra integer constraints can also be added to (\ref{eq:ec_dis}) to make it suitable for unit commitment phase as well.
\fi




\iffalse
\section{Extension to the AC power flows} Maximum line flow changes and optimization (\ref{eq:ec_dis}) can also be computed using the AC power flow equations. %The only difference is that in the AC case, the $\Delta f_{ij}^{\max}(\vec{p_g})$ cannot be computed as simply as in (\ref{eq:max_delta_f}).
To compute the maximum flow changes on the lines under AC power flow equations, one needs to compute the following optimization problem separately for each line $(i,j)$:
\begin{eqnarray*}
&\max_{\Delta s_1,\dots,\Delta s_k} \Delta f_{ij}~~\text{s.t.}&\\
&\Delta \vec{p}=\sum_{l=1}^k \Delta p_l  \vec{w}_l,&\\
&-\Delta p_l^{\max}\leq \Delta p_l\leq \Delta p_l^{\max},&\\
&-\Delta q_l^{\max}\leq \Delta q_l\leq \Delta q_l^{\max},&\\
%&\vec{p}^T.\vec{1}\approx0,&\nonumber\\
&\text{ and AC Power flow equations and constraints},&
\end{eqnarray*}
in which $s_i := p_k+\textbf{i}q_i$ is the apparent power generated by generator $i$. Notice that under the AC power flows, $f_{ij}$ can reflect the apparent power flow on a line instead of only the active power flow.

Optimization above can be very time consuming to solve since it requires solving a nonlinear and nonconvex optimization for every single line in the grid. In order to speed up the process, the approximate line power flow increases can be computed as in (\ref{eq:max_delta_f}) but instead of solving the DCOPF, the ACOPF version of (\ref{eq:ec_dis}) can be solved to compute the dispatches.



The advantage of solving ACOPF, apart from its accuracy, is that it also reflects the \emph{voltage constraints}. Therefore if a MAD attack results in voltage instability (or in the worst case voltage collapse), it can be predicted in the ACOPF and therefore be resolved in the unit commitment problem.
\fi 
